Efficient and Robust Algorithms for Adversarial Linear Contextual Bandits

We consider an adversarial variant of the classic $K$-armed linear contextual bandit problem where the sequence of loss functions associated with each arm are allowed to change without restriction over time. Under the assumption that the $d$-dimensional contexts are generated i.i.d.~at random from a known distributions, we develop computationally efficient algorithms based on the classic Exp3 algorithm. Our first algorithm, RealLinExp3, is shown to achieve a regret guarantee of $\widetilde{O}(\sqrt{KdT})$ over $T$ rounds, which matches the best available bound for this problem. Our second algorithm, RobustLinExp3, is shown to be robust to misspecification, in that it achieves a regret bound of $\widetilde{O}((Kd)^{1/3}T^{2/3}) + \varepsilon \sqrt{d} T$ if the true reward function is linear up to an additive nonlinear error uniformly bounded in absolute value by $\varepsilon$. To our knowledge, our performance guarantees constitute the very first results on this problem setting.

==> misspecification.tex <==
\section{Misspecification}


	We assume that vectors $x_1, x_2, \dots \in \real^d$ are iid and generated from some distribution $D$. Distribution $D$ and sequence $\theta_1, \theta_2, \dots $ are such that $0 \le x^T\theta_t \le 1$ for any $x\sim D$.
	
	Loss of the learner:
	$$L_T = \sum_{t=1}^T x_t^T \theta_{i_t,t},$$
	Loss of the optimal policy $\pi^*$:
	$$L_T^* = \sum_{t=1}^T x_t^T \theta_{\pi^*(x_t),t},$$
	Regret:
	$$ R_T =   L_T - L_T^*. $$
	We assume that covariance matrix $\Sigma$ of $x_t$ is known. We introduce the estimator:
	$$\tilde{\theta}_{i,t} = \frac{1}{p_{t,i}(x_t)} \Sigma^{-1} x_t (x_t^T \theta_{i, t} + \epsilon_{i,t}(x_t)) \II{i_t = i}.$$
	
	Let $\lambda_{min}$ be the minimal eigenvalue of $\Sigma$ and let $\norm{x_t}^2_2 \le \sigma^2$.
	
	\begin{theorem}
		$$ \EE{R_T}  \le T^{2/3}K^{1/3}d^{1/3}(2\sqrt{\ln K} (1 + \epsilon)+2) + 2\epsilon(\sqrt{d} + 1)T .$$
	\end{theorem}
	
	\begin{proof}
	By Lemma~\ref{exp2base}, 
	\begin{align*}
	(1 - \gamma)\EE{- \sum_{t=1}^T \tilde{x}^T \widetilde{\theta}_{\pi^*(\tilde{x}),t} -  \frac{\ln K}{\eta}} \le \EE{ \sum_{t=1}^T  \sum_{i=1}^K p_{i, t}(\tilde{x})   \bigg(  -   
	\tilde{x}^T \widetilde{\theta}_{t,i} + \eta \big( \tilde{x}^T \widetilde{\theta}_{t,i}  
	\big)^2   \bigg) + \frac{\gamma}{K}  
	\tilde{x}^T \widetilde{\theta}_{t,i} }.
	\end{align*}
	First, we consider the first term on the left side. Applying Cauchy–Schwarz inequality,
	\begin{align*}
	&\EE{- \sum_{t=1}^T \tilde{x}^T \widetilde{\theta}_{\pi^*(\tilde{x}),t} }  = \EE{- \sum_{t=1}^T \tilde{x}^T \frac{1}{p_{t,\pi^*(\tilde{x})}(x_t)} \Sigma^{-1} x_t (x_t^T \theta_{\pi^*(\tilde{x}), t} + \epsilon_{t}) \II{i_t(x_t) = \pi^*(\tilde{x})}.} \\
	& = - \sum_{t=1}^T \EE{\EEcc{\tilde{x}^T \frac{1}{p_{t,\pi^*(\tilde{x})}(x_t)} \Sigma^{-1} x_t x_t^T \theta_{\pi^*(\tilde{x}), t} \II{i_t(x_t) = \pi^*(\tilde{x})} }{\tilde{x}}} \\
	& - \EE{ \tilde{x}^T \frac{1}{p_{t,\pi^*(\tilde{x})}(x_t)} \Sigma^{-1} x_t \epsilon_{t} \II{i_t(x_t)  = \pi^*(\tilde{x})}} \\
	& \ge - \sum_{t=1}^T \EE{\tilde{x}^T \theta_{\pi^*(\tilde{x}), t}  } 
	 -   \sqrt{\EE{ \tilde{x}^T \Sigma^{-1} x_t  \tilde{x}^T \Sigma^{-1} x_t }} \cdot \sqrt{\EE{\epsilon_{t}^2}}   .
	\end{align*}
	
	\begin{align*}
	\EE{ \tilde{x}^T \Sigma^{-1} x_t  \tilde{x}^T \Sigma^{-1} x_t }  =  \EE{ x_t x_t^T  \Sigma^{-1} } \EE{\tilde{x} \tilde{x}^T \Sigma^{-1}  } = \trace{I} = d,
	\end{align*}
	Then,
	\begin{align*}
	& - \sum_{t=1}^T \EE{\tilde{x}^T \theta_{\pi^*(\tilde{x}), t}  } 
	-   \sqrt{\EE{ \tilde{x}^T \Sigma^{-1} x_t  \tilde{x}^T \Sigma^{-1} x_t }} \cdot \sqrt{\EE{\epsilon_{t}^2}} \ge - \sum_{t=1}^T \EE{\tilde{x}^T \theta_{\pi^*(\tilde{x}), t}  } 
	-   \epsilon \sqrt{d} \\
	& \ge - \sum_{t=1}^T \EE{\tilde{x}^T \theta_{\pi^*(\tilde{x}), t}  + \epsilon_t} 
	-   \epsilon( \sqrt{d} + 1)   = - \EE{L^*_T} -   \epsilon( \sqrt{d} + 1).
	\end{align*}
	Following the analysis above, 
	
	\begin{align*}
	- \EE{ \sum_{t=1}^T  \sum_{i=1}^K p_{i, t}(\tilde{x})     
	\tilde{x}^T \widetilde{\theta}_{t,i} } &\le - \sum_{t=1}^T \EE{  \sum_{i=1}^K p_{i, t}(\tilde{x})   \tilde{x}^T \theta_{t, i}  }  \\
	& \le - \sum_{t=1}^T \EE{  \sum_{i=1}^K p_{i, t}(\tilde{x}) (  \tilde{x}^T \theta_{t, i} + \epsilon_{i, t }  )} = - \EE{L_T}
    +   \epsilon (\sqrt{d}+1) .
	\end{align*}
	Consider the square term. Since $1/p_{i,t}(x) \le K/\gamma$ and $x_t^T \theta_{t,i} \le 1$,
	\begin{align*}
	& \eta \cdot \EE{ \sum_{t=1}^T  \sum_{i=1}^K p_{i, t}(\tilde{x})    \big( \tilde{x}^T \widetilde{\theta}_{t,i}  \big)^2  } \\
	&  = 	\eta \cdot \EE{ \sum_{t=1}^T  \sum_{i=1}^K p_{i, t}(\tilde{x})  \tilde{x}^T \frac{1}{p^2_{t,i}(x_t)} \Sigma^{-1} x_t (x_t^T \theta_{i, t} + \epsilon_{i,t}(x_t))   \tilde{x}^T  \Sigma^{-1} x_t (x_t^T \theta_{i, t} + \epsilon_{i,t}(x_t)) \II{i_t(x_t) = i}   }  \\
	& \le 	\eta \cdot \EE{ \sum_{t=1}^T  \sum_{i=1}^K p_{i, t}(\tilde{x})   \frac{K}{p_{t,i}(x_t) \gamma} \trace{\Sigma^{-1} x_t x_t^T   \Sigma^{-1} x_t x_t^T } \II{i_t(x_t) = i}   } \\
	& + 2\eta \cdot \EE{ \sum_{t=1}^T  \sum_{i=1}^K p_{i, t}(\tilde{x})   \frac{K}{p_{t,i}(x_t) \gamma} \trace{ \Sigma^{-1} x_t x_t^T     \Sigma^{-1} \tilde{x}\tilde{x}^T } \epsilon_{i,t} \II{i_t(x_t) = i}   } \\
	& + \eta \cdot \EE{ \sum_{t=1}^T  \sum_{i=1}^K p_{i, t}(\tilde{x})  \frac{K}{p_{t,i}(x_t) \gamma} \trace{ \Sigma^{-1}     \tilde{x}\tilde{x}^T  \Sigma^{-1} x_t x_t^T  } \epsilon_{i,t}^2 \II{i_t(x_t) = i}   } \\
	& \le	T \eta K d  (1 + \epsilon)^2 /\gamma.
	\end{align*}
	Summing up all the bounds, we get
	\begin{align*}
	\EE{L_T - L^*_T} \le \gamma T + \frac{\ln K}{\eta} + 2\epsilon(\sqrt{d} + 1)T + T \eta d  (1 + \epsilon)^2\cdot \frac{K}{\gamma} + \gamma \cdot T
	\end{align*}
	With our choice $\eta = T^{-2/3}k^{-1/3}d^{-1/3} \cdot \frac{\sqrt{\ln K}}{ (1+\epsilon)}$, $\gamma = T^{-1/3}k^{1/3}d^{1/3}$, we finally get
	\begin{align*}
	\EE{L_T - L^*_T} \le T^{2/3}K^{1/3}d^{1/3}(2\sqrt{\ln K} (1 + \epsilon)+2) + 2\epsilon(\sqrt{d} + 1)T 
	\end{align*}
	\end{proof}

==> truncation.tex <==
\section{Truncation}

Distribution $D$ is such that  $\twonorm{x_t}^2 \le \sigma^2$.

At each round $t$, we have access to the distribution $D$, and during each time step $t$ we perform Geometric resampling :

For $k = 1, \dots, M$:
\begin{itemize}
	\item sample $x(k) \sim D$, $i_k \sim p_{i, t}(x(k))$
	\item $B_{k,i} = x(k)x(k)^T\II{i_k = i}$
\end{itemize}

Let $A_{k,i} = \prod_{j=0}^k  (I - \beta B_{j,i}) $, then introduce an estimator:
$$\widehat{\Sigma}^{-1}_{t,i,M} = \beta \sum_{k=0}^M A_{k,i}  .$$

Where we assume that $\beta < \frac{1}{2 \sigma^2}$.

Now we define an estimator:
$$\widehat{\theta}_{i,t} = \widehat{\Sigma}^{-1}_{t,i,M} x_t x_t^T \theta_{t,i} \II{i_t(x_t )= i}.$$


\redd{put it later somewhere}
Note, that $\Sigma_{t,i}^{-1} = \beta \sum_{j=0}^{\infty} (I - \beta \Sigma_{t,i})^j$.
Then,
\begin{align*}
\Sigma^{-1}_{t,i,M}  = \EE{\widehat{\Sigma}^{-1}_{t,i,M} } = \Sigma_{t,i}^{-1} - (I - \beta \Sigma_{t,i})^M \Sigma_{t,i}^{-1} .
\end{align*}


\begin{algorithm}[H]
	\caption{ Contextual Exp3 2}
	\label{alg:thealg2}
	\textbf{Parameters:}  real numbers $\eta, \gamma \in (0,1)$.\\
	\textbf{Initialization:} play $i_1$ uniformly at random from  $ 1,\dots, K$.
	\\
	\textbf{For} $t = 2, \dots, T$, \textbf{repeat}
	\begin{enumerate}
		\item observe $x_t$, set 
		$$w_{i,t}(x_t) = \exp\bigg(- \eta  x_t^T\sum_{s=1}^{t-1} \widehat{\theta }_{i,s}  \bigg),$$
		\item draw $i_t$ with probability $$  p_{i,t}(x_t)= (1-\gamma) \frac{w_{i,t}(x_t)}{\sum_i w_{i,t}(x_t)} + \frac{\gamma}{K} , $$
		\item receive reward $x_t^T \theta_{i_t, t}$,
		\item get $\Sigma^{-1}_{t,i,M}$, $\widehat{\theta }_{i,t}$ for all $i$.
	\end{enumerate}
\end{algorithm}

The proof of the following statement follows the standard argument for Exp3, see, for example \cite{AuerCFS02}. For the sake of completeness, we include proof in the appendix.

We prove the following bound on the regret of the Algorithm~\ref{alg:thealg2}:
\begin{theorem}
	$$ \EE{L_T} - \EE{L^*_T} \le 4\sqrt{T}  + 2\sqrt{TK \ln K } \sqrt{\frac{\trace{\Sigma} + d}{\beta(2-\beta \sigma^2)}  }.$$
\end{theorem}

\begin{proof}
	By Lemma~\ref{exp2base}, 
	\begin{align*}
	(1 - \gamma)\EE{- \sum_{t=1}^T \tilde{x}^T \widehat{\theta}_{\pi^*(\tilde{x}),t} -  \frac{\ln K}{\eta}} \le \EE{ \sum_{t=1}^T  \sum_{i=1}^K p_{i, t}(\tilde{x})   \bigg(  -   
		\tilde{x}^T \widehat{\theta}_{t,i} + \eta \big( \tilde{x}^T \widehat{\theta}_{t,i}  
		\big)^2   \bigg) + \frac{\gamma}{K}  
		\tilde{x}^T \widehat{\theta}_{t,i} }.
	\end{align*}
	First, we consider the first term on the left side. By Lemma~\ref{linear_term}, 
		\begin{align*}
	- \sum_{t=1}^T \EE{  \tilde{x}^T \widehat{\theta}_{t, \pi^*(\tilde{x})}  }
	= 	-\EE{L_T^*} + \sum_{t=1}^T  \EE{\tilde{x}^T(I - \beta \Sigma_{t,\pi^*(\tilde{x})})^M \theta_{t,\pi^*(\tilde{x})}  }. 
	\end{align*}
	By Lemma~\ref{trace_M} and since $\tilde{x}^T  \theta_{t,i} \ge -1 $ almost surely,
	\begin{align*}
	- \EE{L_T^*}+ \sum_{t=1}^T  \EE{\tilde{x}^T(I - \beta \Sigma_{t,i})^M \theta_{t,\pi^*(\tilde{x})}  }  \ge  -\EE{L_T^*}  - \sqrt{T}.
	\end{align*}
	In the same way, by Lemma~\ref{linear_term}, Lemma~\ref{trace_M} and since $\tilde{x}^T  \theta_{t,i} \le 1 $ almost surely,
	\begin{align*}
	- \sum_{t=1}^T  \sum_{i=1}^K \EE{  p_{i, t}(\tilde{x}) \tilde{x}^T \widehat{\theta}_{t,i}} \le - \EE{L_T} + \sqrt{T}
	\end{align*}
	The proof we are left with is bounding the quadratic term. By Lemma~\ref{quadratic}, 
	$$\EEtt{\sum_{i=1}^K p_{i,t}(\tilde{x})(\tilde{x}^T\widehat{\theta}_{t,i})^2} \le K \cdot \frac{\trace{\Sigma} + d}{\beta(2-\beta \sigma^2)} ,$$
	where we assume that $\beta < 1/2 \sigma^2$. In result, with $\gamma = 1/\sqrt{T}$, $\eta =\sqrt{\frac{\ln K}{K}}\cdot \sqrt{\frac{\beta(2-\beta \sigma^2)}{\trace{\Sigma} + d} }$, we get
	$$ \EE{L_T} - \EE{L^*_T} \le 4\sqrt{T}  + 2\sqrt{TK \ln K } \sqrt{\frac{\trace{\Sigma} + d}{\beta(2-\beta \sigma^2)}  }.$$
\end{proof}




==> truncation_proof.tex <==
\section{The proof of Theorem \ref{exp3regret}}

\begin{lemma}
	\label{linear_term}
	\begin{align*}
	\EE{\sum_{i=1}^K p_{i, t}(\tilde{x})  \tilde{x}^T\widehat{\theta}_{t,i}}
	&= 	\EE{\tilde{x}^T  \theta_{t,i}  } - \EE{\tilde{x}^T(I - \beta \Sigma_{t,i})^M \theta_{t,i}  } 
	\end{align*}
\end{lemma}
   
\begin{proof}
	First, note that
	\begin{align*}
	\EE{ \sum_{i=1}^K p_{i, t}(\tilde{x})  \tilde{x}^T\widehat{\theta}_{t,i}}
	&= \EE{\sum_{i=1}^K p_{i, t}(\tilde{x})  \tilde{x}^T\widehat{\Sigma}^{+}_{t,i,M} x_t x_t^T \theta_{t,i} \II{i_t(x_t )= i} }  \\
	& =  \EE{\sum_{i=1}^K p_{i, t}(\tilde{x})  \tilde{x}^T\EE{\widehat{\Sigma}^{+}_{t,i,M} x_t x_t^T \II{i_t(x_t )= i} | \tilde{x} } \theta_{t,i}  } \\
	&= \EE{\sum_{i=1}^K p_{i, t}(\tilde{x})  \tilde{x}^T\EE{\widehat{\Sigma}^{+}_{t,i,M} } \EE{x_t x_t^T \II{i_t(x_t )= i} }   \theta_{t,i}  }  \\
	&=\EE{\sum_{i=1}^K p_{i, t}(\tilde{x}) \tilde{x}^T\EE{\widehat{\Sigma}^{+}_{t,i,M} } \Sigma_{t,i}  \theta_{t,i}  }. 
	\end{align*}
	Where the last equations follows by independence of $x_t$ and $x(1), \dots, x(k)$. Since   $x(1), \dots x(k)$ are i.i.d.,
	\begin{align*}
	  \EE{\widehat{\Sigma}^{+}_{t,i,M} } =  \beta \big(I + \sum_{k=1}^M \big(I - \beta\Sigma_{t,i} \big)^k  \big) = \Sigma_{t,i}^{-1} - (I - \beta \Sigma_{t,i})^M \Sigma_{t,i}^{-1}.
	\end{align*}
	Then we get 
	\begin{align*}
	\EE{\sum_{i=1}^K p_{i, t}(\tilde{x}) \tilde{x}^T\widehat{\theta}_{t,i}}
	&= 	\EE{\sum_{i=1}^K p_{i, t}(\tilde{x}) \tilde{x}^T  \theta_{t,i}  } - \EE{\sum_{i=1}^K p_{i, t}(\tilde{x}) \tilde{x}^T(I - \beta \Sigma_{t,i})^M \theta_{t,i}  } 
	\end{align*}
		
\end{proof}

Considering the second term, since $\tilde{x}^T  \theta_{t,i} \ge -1 $ almost surely,
\begin{align*}
- \EE{\tilde{x}^T(I - \beta \Sigma_{t,i})^M \theta_{t,i}  } 
\le tr\big( (I - \beta \Sigma_{t,i})^M \big). \\
\end{align*}

\begin{lemma}
	\label{trace_M}
	For any 
	$
	M \ge \frac{\log (\sqrt{T}) K}{\gamma \beta \lambda_{min}\pa{\Sigma}},
	$ we have
	$$ tr\bigg((I - \beta \Sigma_{t,i})^M  \bigg) 
	\le  \frac{1}{\sqrt{T}}. $$
\end{lemma}
\begin{proof}
	Let $i'(x(k))$ be the arm sampled from the distribution $p'_{i'}(x(k)) = \frac{w_{i',t}(x(k))}{W_{t}(x(k))}$, then such sampling generates the covariance matrix $\Sigma'_{t,i} = \EE{xx^T \II{i'(x) = i}  }$.  Then we can write $\Sigma_{t,i}$ as a sum: 
	$$ \Sigma_{t,i} = \big(1-\frac{\gamma}{K}\big)\Sigma'_{t,i} + \frac{\gamma}{K} \Sigma, $$
	Since $\Sigma$, $\Sigma_{t,i}$ and $\Sigma'_{t,i}$ are positive semi-definite matrices, and we denote the minimal eigenvalue by $\lambda_{min}$, then $$\lambda_{min}\pa{\Sigma_{t,i}} \ge \frac{\gamma}{K} \lambda_{min}\pa{\Sigma} + (1-\frac{\gamma}{K}) \lambda_{min}\pa{\Sigma'_{t,i}} \ge \frac{\gamma}{K} \lambda_{min}\pa{\Sigma} $$
	Then,
	$$ tr\bigg((I - \beta \Sigma_{t,i})^M  \bigg) 
	\le \pa{1-\frac{\gamma \beta}{K} \lambda_{min}\pa{\Sigma} }^M $$
	Using the inequality $e^{-x} \ge 1-x$,
	we get
	$$\pa{1-\frac{\gamma \beta}{K} \lambda_{min}\pa{\Sigma} }^M \le \exp\pa{ -\frac{\gamma \beta}{K} \lambda_{min}\pa{\Sigma} M} \le \frac{1}{\sqrt{T}}.  $$
\end{proof}


\subsection{Bounding the quadratic term}
For 
simplicity, we let $\beta = 1$ and will play around with its value to ensure the conditions 
that will pop up later. 

\begin{lemma}
	\label{quadratic}
	For any 
	$$\EEtt{\sum_{i=1}^K p_{i,t}(\tilde{x})(\tilde{x}^T\widehat{\theta}_{t,i})^2} \le K \cdot \frac{\trace{\Sigma} + d}{\beta(2-\beta \sigma^2)} .$$
\end{lemma}
\begin{proof}

\begin{align*}
&\EEtt{\sum_{i = 1}^K p_{t,i}(\tx) \pa{\tx\transpose \Sp_{t,i} x_t x_t\transpose\theta_{t,i} \II{I_t=i}}^2} 
\le \EEtt{\sum_{i = 1}^K  \trace{p_{t,i}(\tx) \tx\tx\transpose \Sp_{t,i} x_t x_t\transpose \Sp_{t,i} 
		\II{I_t=i}}}
\\
&= \sum_{i = 1}^K   \EEtt{ \trace{\Sigma_{t,i} \Sp_{t,i} \Sigma_{t,i} \Sp_{t,i}} }.
\end{align*}
In what follows, we suppress the $t,i$ indexes for ease of readability. Using the definition of 
$\Sp$, we have
\begin{align*}
\EE{\trace{\Sigma \Sigma^+ \Sigma \Sigma^+}} &= \EE{\trace{\Sigma \pa{\sum_{k=0}^M A_k} \Sigma 
		\pa{\sum_{j=0}^M A_j}}}
\\
&= \sum_{k=0}^M \sum_{j=0}^M\trace{ \EE{\Sigma A_k \Sigma A_j}} 
= 
\sum_{k=0}^M \trace{\EE{\Sigma A_k \Sigma A_k}} + 2\sum_{k=0}^M \sum_{j= k+1}^M \trace{\EE{\Sigma 
		A_k \Sigma A_j}}.
\end{align*}
Considering the first term, we notice that 
\begin{align*}
\EE{(I- \beta B_k) \Sigma (I - \beta B_k)} &= \EE{(I - \beta x_kx_k\transpose) \Sigma (I - 
	\beta x_kx_k\transpose)} 
= \Sigma - \beta\EE{x_kx_k\transpose\Sigma} - \beta\EE{\Sigma x_kx_k\transpose} 
\\
& + \beta^2 \EE{x_kx_k\transpose \Sigma x_kx_k\transpose} \preccurlyeq \Sigma - 2\beta \Sigma^2  + \beta^2 \sigma^2 \Sigma^2 = \Sigma \pa{I - \beta (2-\beta\sigma^2)\Sigma},
\end{align*}
\redd{add assumptions in the section}
\redd{if we assume that the moment condition $\EE{\twonorm{x_k}^2 x_kx_k\transpose} \preccurlyeq 
	\sigma^2 \Sigma$ holds, which is actually true when $\twonorm{x_k}^2 \le \sigma^2$ holds almost 
	surely. The condition $\sigma^2 \le 2$ can be ensured by an appropriate choice of $\beta$.} Now, 
using the above relation recursively, we get
\[
\trace{\EE{\Sigma A_k \Sigma A_k} }= \trace{\EE{\Sigma A_{k-1} \EE{(I - \beta B_k) \Sigma (I- \beta B_k)}A_{k-1}}} = \trace{\Sigma^2 (I - 
\beta (2-\beta \sigma^2)\Sigma)^{k}},
\]
we can see that
\begin{align*}
\sum_{k=0}^M \trace{\Sigma^2 (I - 
	\beta (2-\beta \sigma^2)\Sigma)^{k}} = \frac{1}{\beta(2-\beta\sigma^2)} \trace{\Sigma^2 \Sigma^{-1} \pa{I - (I - 
		\beta(2-\beta \sigma^2)\Sigma)^M}} \le \frac{\trace{\Sigma}}{\beta(2-\beta \sigma^2)}.
\end{align*}
Now, regarding the second term, we have
\begin{align*}
\sum_{k=0}^M \sum_{j= k+1}^M \EE{\trace{\Sigma A_k \Sigma A_j}} 
&= \sum_{k=0}^M \EE{\EEcc{\sum_{j= k+1}^M \trace{\Sigma A_k \Sigma A_j}}{B_1,B_2,\dots,B_k}}
\\
&= \sum_{k=0}^M \EE{\EEcc{\sum_{j= k+1}^M \trace{\Sigma A_k \Sigma A_k (I - 
			\Sigma)^{j-k}}}{B_1,B_2,\dots,B_k}}
\\
&= \sum_{k=0}^M \EE{\EEcc{\trace{\Sigma A_k \Sigma A_k \Sigma^{-1}\pa{I - (I - 
				\Sigma)^{M-k}}}}{B_1,B_2,\dots,B_k}}
\\
&\le \sum_{k=0}^M \EE{\EEcc{\trace{\Sigma A_k \Sigma A_k \Sigma^{-1}}}{B_1,B_2,\dots,B_k}}
\\
&= \frac{1}{\beta(2-\beta \sigma^2)} \EE{\trace{\Sigma^2 \Sigma^{-1} \pa{I - (I - 
			\beta(2-\beta \sigma^2)\Sigma)^M \Sigma^{-1}}}} 
\\
&\le \frac{1}{\beta(2-\beta \sigma^2)} \EE{\trace{\Sigma^2 \Sigma^{-1} \Sigma^{-1}}} \le \frac{d}{\beta(2-\beta \sigma^2)}.
\end{align*}

\end{proof}
